Leveraging Uncertainties to Infer Preferences: Robust Analysis of School Choice

Inferring applicant preferences is fundamental in many analyses of school-choice data. Application mistakes make this task challenging. We propose a novel approach to deal with the mistakes in a deferred-acceptance matching environment. The key insight is that the uncertainties faced by applicants, e.g., due to tie-breaking lotteries, render some mistakes costly, allowing us to reliably infer relevant preferences. Our approach extracts all information on preferences robustly to payoff-insignificant mistakes. We apply it to school-choice data from Staten Island, NYC. Counterfactual analysis suggests that we underestimate the effects of proposed desegregation reforms when applicants' mistakes are not accounted for in preference inference and estimation.

==> tables/cf_aggregate.tex <==
\begin{table}[htbp]
	\caption{Aggregate Segregation Measures in Staten Island\label{tab:cf_aggregate}}
	\centering\footnotesize
	\begin{tabular}{lrcccc}
		\toprule
		&&(1)&(2)&(3)&(4)\\
		& \multicolumn{1}{l}{} & Data & No Screening & No Zoned & No Priority \\\midrule
		\multicolumn{6}{l}{\textit{Panel A: Theil's H Index}}                                            \\
		& WTT                  & 0.18 & 0.16         & 0.17     & 0.16        \\
		& TEPS                 &      & 0.15         & 0.11     & 0.10        \\
		& STB                  &      & 0.15         & 0.10     & 0.09        \\
		& Selected             &      & 0.15         & 0.11     & 0.09        \\
		\multicolumn{6}{l}{\textit{Panel B: Sorting Indices}}                                            \\
		Sorting by Race   & WTT                  & 0.26 & 0.25         & 0.26     & 0.24        \\
		& TEPS                 &      & 0.24         & 0.16     & 0.14        \\
		& STB                  &      & 0.24         & 0.16     & 0.14        \\
		& Selected             &      & 0.24         & 0.16     & 0.14        \\
		&&&&&\\
		Sorting by Income & WTT                  & 0.29 & 0.27         & 0.28     & 0.27        \\
		& TEPS                 &      & 0.27         & 0.17     & 0.15        \\
		& STB                  &      & 0.26         & 0.16     & 0.14        \\
		& Selected             &      & 0.27         & 0.16     & 0.15        \\
		\bottomrule
	\end{tabular}
\end{table}

==> tables/desc_2panels.tex <==
\begin{table}[h!]
\centering
\caption{Comparing Preferences Inferred by Stability, TEPS, and WTT: Regressions \label{tab:stb_2panels}}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\resizebox{0.95\textwidth}{!}{\begin{tabular}{l*{8}{c}}
\toprule            &\multicolumn{1}{c}{Cell 1}&\multicolumn{1}{c}{Cell 2}&\multicolumn{1}{c}{Cell 3}&\multicolumn{1}{c}{Cell 4}&\multicolumn{1}{c}{Cell 5}&\multicolumn{1}{c}{Cell 6}&\multicolumn{1}{c}{Cell 7}&\multicolumn{1}{c}{Cell 8}\\
\midrule
\multicolumn{9}{l}{\it Panel A: Stability versus TEPS} \\
[0.25em]
Inferred by stability     &      -0.038         &      -0.486         &       1.590         &       0.356         &       7.706\sym{***}&       1.926         &       1.919         &       3.628\sym{***}\\
            &     (1.574)         &     (1.299)         &     (1.736)         &     (1.783)         &     (1.858)         &     (3.402)         &     (1.303)         &     (1.134)         \\
[0.25em]
Distance to program~$j_1$ &      -0.338         &      -3.256\sym{***}&      -1.728         &      -4.392\sym{**} &       0.038         &      -0.253         &       0.327         &       1.047         \\
            &     (1.218)         &     (1.205)         &     (1.756)         &     (1.792)         &     (1.486)         &     (1.230)         &     (1.219)         &     (0.757)         \\
[0.25em]
Distance to program~$j_2$  &       1.521\sym{***}&       1.683\sym{***}&       0.779\sym{***}&       1.094\sym{***}&       0.121         &      -0.023         &      -0.368\sym{***}&      -0.464\sym{***}\\
            &     (0.108)         &     (0.098)         &     (0.135)         &     (0.136)         &     (0.224)         &     (0.345)         &     (0.101)         &     (0.114)         \\
[0.25em]
Program~$j_1$ is $i$'s nearest &       5.529         &       0.270         &       3.601         &      -6.015         &      -3.782         &       1.150         &      -2.883         &       2.084         \\
            &     (4.257)         &     (3.501)         &     (5.005)         &     (5.231)         &     (5.046)         &     (8.981)         &     (4.909)         &     (4.041)         \\
[0.25em]
Program~$j_2$ is $i$'s nearest &       1.692\sym{***}&       1.007\sym{**} &       0.518         &       1.966\sym{***}&       0.331         &       1.510\sym{*}  &      -0.504\sym{*}  &      -0.839\sym{***}\\
            &     (0.572)         &     (0.488)         &     (0.569)         &     (0.595)         &     (0.546)         &     (0.843)         &     (0.291)         &     (0.282)         \\
[0.25em]
Intercept      &      12.165\sym{***}&      22.594\sym{***}&      13.612\sym{**} &      24.074\sym{***}&       3.073         &      13.353\sym{**} &       3.729         &      -1.264         \\
            &     (4.673)         &     (4.201)         &     (5.665)         &     (6.214)         &     (4.634)         &     (5.388)         &     (4.294)         &     (2.740)         \\
[0.25em]
\(N\)       &       34890         &       36854         &       23663         &       24608         &        8884         &        6724         &       26767         &       24535         \\
[0.75em]
\multicolumn{9}{l}{\it Panel B: Stability versus WTT} \\
[0.25em]
Inferred by stability  &       4.807\sym{***}&       6.415\sym{***}&       7.039\sym{***}&       4.505\sym{***}&       8.838\sym{***}&       7.954\sym{***}&       6.780\sym{***}&       6.183\sym{***}\\
            &     (1.215)         &     (1.218)         &     (1.426)         &     (1.492)         &     (1.809)         &     (2.339)         &     (1.037)         &     (0.936)         \\
[0.25em]
Distance to program~$j_1$ &      -0.034         &       1.338         &       1.031         &      -0.564         &       0.545         &       2.071\sym{*}  &       3.665\sym{***}&       2.277\sym{***}\\
            &     (0.755)         &     (0.889)         &     (0.868)         &     (0.989)         &     (1.227)         &     (1.221)         &     (0.659)         &     (0.600)         \\
[0.25em]
Distance to program~$j_2$ &       2.015\sym{***}&       2.130\sym{***}&       0.581\sym{**} &       1.139\sym{***}&      -2.768\sym{***}&      -2.458\sym{***}&      -3.765\sym{***}&      -4.048\sym{***}\\
            &     (0.196)         &     (0.188)         &     (0.292)         &     (0.290)         &     (0.418)         &     (0.480)         &     (0.179)         &     (0.171)         \\
[0.25em]
Program~$j_1$ is $i$'s nearest &      -6.268\sym{**} &       6.100\sym{**} &      -2.374         &     -12.523\sym{***}&      -6.254\sym{*}  &      -7.442\sym{*}  &      -0.156         &      -3.884\sym{**} \\
            &     (2.673)         &     (2.879)         &     (3.198)         &     (2.994)         &     (3.204)         &     (4.443)         &     (1.944)         &     (1.948)         \\
[0.25em]
Program~$j_2$ is $i$'s nearest &       2.846\sym{***}&       3.017\sym{***}&       0.906         &       2.339\sym{**} &      -1.175         &      -0.467         &      -2.940\sym{***}&      -3.438\sym{***}\\
            &     (0.796)         &     (0.790)         &     (0.887)         &     (1.002)         &     (0.896)         &     (1.395)         &     (0.397)         &     (0.458)         \\
[0.25em]
Intercept      &      13.927\sym{***}&       4.591         &       8.835\sym{***}&      15.335\sym{***}&      11.586\sym{***}&      13.711\sym{***}&       1.923         &       7.006\sym{***}\\
            &     (2.641)         &     (3.009)         &     (2.747)         &     (3.262)         &     (3.310)         &     (4.067)         &     (2.048)         &     (1.925)         \\
[0.25em]
\(N\)       &      122242         &      128121         &       78423         &       82659         &       38168         &       27826         &      116400         &      111635         \\
\bottomrule
\end{tabular}}
	\begin{tabnotes}
Each observation is a binary relation, $j$, which specifies that program~$j_1$ is more preferred than $j_2$, inferred for student~$i$ by TEPS in panel~A and by WTT in panel~B. The dependent variable is the difference in the percentage of high-performing students between $j_1$ and $j_2$. A student is a high performer if her average of ELA and math scores is above the 75th percentile among all students. Student fixed effects are included. Standard errors in parentheses are clustered at the student-level.  * $p<0.1$, ** $p<0.05$, *** $p<0.01$.
	\end{tabnotes}
\end{table}


==> tables/desc_teps.tex <==
\begin{table}[h!]
\centering
\caption{Comparing Preferences Inferred by Stability and TEPS: Regression Results \label{tab:stb_teps}}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\resizebox{0.95\textwidth}{!}{\begin{tabular}{l*{8}{c}}
\toprule            &\multicolumn{1}{c}{Cell 1}&\multicolumn{1}{c}{Cell 2}&\multicolumn{1}{c}{Cell 3}&\multicolumn{1}{c}{Cell 4}&\multicolumn{1}{c}{Cell 5}&\multicolumn{1}{c}{Cell 6}&\multicolumn{1}{c}{Cell 7}&\multicolumn{1}{c}{Cell 8}\\
\midrule
Inferred by stability     &      -0.038         &      -0.486         &       1.590         &       0.356         &       7.706\sym{***}&       1.926         &       1.919         &       3.628\sym{***}\\
            &     (1.574)         &     (1.299)         &     (1.736)         &     (1.783)         &     (1.858)         &     (3.402)         &     (1.303)         &     (1.134)         \\
[0.25em]
Distance to program~$j_1$ &      -0.338         &      -3.256\sym{***}&      -1.728         &      -4.392\sym{**} &       0.038         &      -0.253         &       0.327         &       1.047         \\
            &     (1.218)         &     (1.205)         &     (1.756)         &     (1.792)         &     (1.486)         &     (1.230)         &     (1.219)         &     (0.757)         \\
[0.25em]
Distance to program~$j_2$  &       1.521\sym{***}&       1.683\sym{***}&       0.779\sym{***}&       1.094\sym{***}&       0.121         &      -0.023         &      -0.368\sym{***}&      -0.464\sym{***}\\
            &     (0.108)         &     (0.098)         &     (0.135)         &     (0.136)         &     (0.224)         &     (0.345)         &     (0.101)         &     (0.114)         \\
[0.25em]
Program~$j_1$ is $i$'s nearest &       5.529         &       0.270         &       3.601         &      -6.015         &      -3.782         &       1.150         &      -2.883         &       2.084         \\
            &     (4.257)         &     (3.501)         &     (5.005)         &     (5.231)         &     (5.046)         &     (8.981)         &     (4.909)         &     (4.041)         \\
[0.25em]
Program~$j_2$ is $i$'s nearest &       1.692\sym{***}&       1.007\sym{**} &       0.518         &       1.966\sym{***}&       0.331         &       1.510\sym{*}  &      -0.504\sym{*}  &      -0.839\sym{***}\\
            &     (0.572)         &     (0.488)         &     (0.569)         &     (0.595)         &     (0.546)         &     (0.843)         &     (0.291)         &     (0.282)         \\
[0.25em]
Intercept      &      12.165\sym{***}&      22.594\sym{***}&      13.612\sym{**} &      24.074\sym{***}&       3.073         &      13.353\sym{**} &       3.729         &      -1.264         \\
            &     (4.673)         &     (4.201)         &     (5.665)         &     (6.214)         &     (4.634)         &     (5.388)         &     (4.294)         &     (2.740)         \\
\hline
\(N\)       &       34890         &       36854         &       23663         &       24608         &        8884         &        6724         &       26767         &       24535         \\
\bottomrule
\end{tabular}}
	\begin{tabnotes}
Each observation is a binary relation, $j$, which specifies that program~$j_1$ is more preferred than $j_2$, inferred by TEPS for student~$i$. The dependent variable is the difference in the percentage of high-performing students between $j_1$ and $j_2$. A student is a high performer if her average of ELA and math scores is above the 75th percentile among all students. Student fixed effects are included. Standard errors in parentheses are clustered at the student-level.  * $p<0.1$, ** $p<0.05$, *** $p<0.01$.
	\end{tabnotes}
\end{table}


==> tables/desc_wtt.tex <==
\begin{table}[h!]
\centering
\caption{Comparing Preferences Inferred by Stability and WTT: Regression Results\label{tab:stb_wtt}}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\resizebox{0.95\textwidth}{!}{\begin{tabular}{l*{8}{c}}
\toprule            &\multicolumn{1}{c}{Cell 1}&\multicolumn{1}{c}{Cell 2}&\multicolumn{1}{c}{Cell 3}&\multicolumn{1}{c}{Cell 4}&\multicolumn{1}{c}{Cell 5}&\multicolumn{1}{c}{Cell 6}&\multicolumn{1}{c}{Cell 7}&\multicolumn{1}{c}{Cell 8}\\
\midrule
Inferred by stability  &       4.807\sym{***}&       6.415\sym{***}&       7.039\sym{***}&       4.505\sym{***}&       8.838\sym{***}&       7.954\sym{***}&       6.780\sym{***}&       6.183\sym{***}\\
            &     (1.215)         &     (1.218)         &     (1.426)         &     (1.492)         &     (1.809)         &     (2.339)         &     (1.037)         &     (0.936)         \\
[0.25em]
Distance to program~$j_1$ &      -0.034         &       1.338         &       1.031         &      -0.564         &       0.545         &       2.071\sym{*}  &       3.665\sym{***}&       2.277\sym{***}\\
            &     (0.755)         &     (0.889)         &     (0.868)         &     (0.989)         &     (1.227)         &     (1.221)         &     (0.659)         &     (0.600)         \\
[0.25em]
Distance to program~$j_2$ &       2.015\sym{***}&       2.130\sym{***}&       0.581\sym{**} &       1.139\sym{***}&      -2.768\sym{***}&      -2.458\sym{***}&      -3.765\sym{***}&      -4.048\sym{***}\\
            &     (0.196)         &     (0.188)         &     (0.292)         &     (0.290)         &     (0.418)         &     (0.480)         &     (0.179)         &     (0.171)         \\
[0.25em]
Program~$j_1$ is $i$'s nearest &      -6.268\sym{**} &       6.100\sym{**} &      -2.374         &     -12.523\sym{***}&      -6.254\sym{*}  &      -7.442\sym{*}  &      -0.156         &      -3.884\sym{**} \\
            &     (2.673)         &     (2.879)         &     (3.198)         &     (2.994)         &     (3.204)         &     (4.443)         &     (1.944)         &     (1.948)         \\
[0.25em]
Program~$j_2$ is $i$'s nearest &       2.846\sym{***}&       3.017\sym{***}&       0.906         &       2.339\sym{**} &      -1.175         &      -0.467         &      -2.940\sym{***}&      -3.438\sym{***}\\
            &     (0.796)         &     (0.790)         &     (0.887)         &     (1.002)         &     (0.896)         &     (1.395)         &     (0.397)         &     (0.458)         \\
[0.25em]
Intercept      &      13.927\sym{***}&       4.591         &       8.835\sym{***}&      15.335\sym{***}&      11.586\sym{***}&      13.711\sym{***}&       1.923         &       7.006\sym{***}\\
            &     (2.641)         &     (3.009)         &     (2.747)         &     (3.262)         &     (3.310)         &     (4.067)         &     (2.048)         &     (1.925)         \\
\hline
\(N\)       &      122242         &      128121         &       78423         &       82659         &       38168         &       27826         &      116400         &      111635         \\
\bottomrule
\end{tabular}}
	\begin{tabnotes}
Each observation is a binary relation, $j$, which specifies that program~$j_1$ is more preferred than $j_2$, inferred by WTT for student~$i$. The dependent variable is the difference in the percentage of high-performing students between $j_1$ and $j_2$. A student is a high performer if her average of ELA and math scores is above the 75th percentile among all students. Student fixed effects are included. Standard errors in parentheses are clustered at the student-level.  * $p<0.1$, ** $p<0.05$, *** $p<0.01$.
	\end{tabnotes}
\end{table}


